On Large Language Models in Mission-Critical IT Governance: Are We Ready Yet?

Context. The security of critical infrastructure has been a pressing concern since the advent of computers and has become even more critical in today's era of cyber warfare. Protecting mission-critical systems (MCSs), essential for national security, requires swift and robust governance, yet recent events reveal the increasing difficulty of meeting these challenges. Aim. Building on prior research showcasing the potential of Generative AI (GAI), such as Large Language Models, in enhancing risk analysis, we aim to explore practitioners' views on integrating GAI into the governance of IT MCSs. Our goal is to provide actionable insights and recommendations for stakeholders, including researchers, practitioners, and policymakers. Method. We designed a survey to collect practical experiences, concerns, and expectations of practitioners who develop and implement security solutions in the context of MCSs. Conclusions and Future Works. Our findings highlight that the safe use of LLMs in MCS governance requires interdisciplinary collaboration. Researchers should focus on designing regulation-oriented models and focus on accountability; practitioners emphasize data protection and transparency, while policymakers must establish a unified AI framework with global benchmarks to ensure ethical and secure LLMs-based MCS governance.

==> Tables/questionaire.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\centering
\caption{Questionaire Questions}
\label{tab:qq}
\resizebox{0.5\linewidth}{!}{%
\begin{tabular}{p{05\linewidth}}
\hline
\multicolumn{1}{c}{\textbf{Demographic Information}}                                                                                                         \\ \hline
1. How old are you?                                                                                                                                          \\
2. How do you identify in terms of gender, if you're comfortable sharing?                                                                                    \\
3. Education Level                                                                                                                                           \\
4. Occupation                                                                                                                                                \\
5. Industry Sector                                                                                                                                           \\
6. Organization Size                                                                                                                                         \\
7. Primary Role in Organization                                                                                                                              \\
8. Years of Experience                                                                                                                                       \\
9. Primary Area of Interest or Expertise                                                                                                                     \\
10. Geographical Location                                                                                                                                    \\ \hline
\multicolumn{1}{c}{\textbf{Familiarity and Usage of LLMs}}                                                                                                   \\ \hline
11. How familiar are you with large language models (LLMs) such as ChatGPT (GPT-3/4), BERT et simila?                                                        \\
12. Have you ever used LLMs specifically for data or risk analysis (even if not IT-related)?                                                                 \\
13. What did you use it for?                                                                                                                                 \\ \hline
\multicolumn{1}{c}{\textbf{Perceptions of LLMs in Security Risk Analysis}}                                                                                   \\ \hline
14. How do you envision LLMs enhancing security risk analysis within mission-critical IT-governance contexts? (Multiple Choice)                              \\
15. In what specific ways do you envision LLMs enhancing security risk analysis within mission-critical IT-governance contexts? (Open Ended)                 \\
16. How would you rate the current capabilities of LLMs in addressing the specific security challenges faced by mission-critical IT-governance environments? (Multiple Choice) \\
17. What are the potential limitations or drawbacks of relying on LLMs for security risk analysis in mission-critical contexts? (Open Ended)                 \\
18. Do you agree with the following sentence? ”Integrating LLMs into existing security risk analysis frameworks is easy.” (Yes/No)                           \\
19. What are your perceptions of integrating LLMs into existing security risk analysis frameworks? (Open Ended)                                              \\
20. Do you agree with the following sentence? ”There are no concerns in integrating LLMs in mission-critical risk analysis.” (Yes/No)                        \\
21. What concerns, if any, do you have regarding using LLMs in mission-critical IT governance environments? (Open Ended)                                     \\
22. To what extent do you believe the adoption of LLMs in mission-critical IT governance will improve overall operational efficiency and effectiveness? (Scale) \\
23. To what extent do you believe the adoption of LLMs in mission-critical IT governance will improve overall operational effectiveness? (Scale)             \\
24. How confident are you in the ability of LLMs to handle and analyze sensitive or classified information securely? (Scale)                                 \\
25. How do you feel about utilizing LLMs to handle sensitive or classified information? (Open Ended)                                                         \\ \hline
\multicolumn{1}{c}{\textbf{Addressing Biases, Ethics, and Privacy Concerns}}                                                                                 \\ \hline
26. What measures should be implemented to address potential biases or ethical concerns associated with LLM adoption in security risk analysis? (Multiple Choice) \\
27. What measures should be implemented to address potential biases or ethical concerns associated with LLM adoption in security risk analysis? (Open Ended) \\
28. How do you perceive the potential impact of LLM adoption on privacy rights and data protection within mission-critical IT governance environments? (Multiple Choice) \\
29. How do you perceive the potential impact of LLM adoption on privacy rights and data protection within mission-critical IT governance environments? (Open Ended) \\ \hline
\multicolumn{1}{c}{\textbf{Regulatory and Policy Measures}}                                                                                                  \\ \hline
30. What regulatory measures are necessary to ensure LLMs' safe and ethical use in mission-critical IT governance? (Multiple Choice)                         \\
31. What regulatory measures are necessary to ensure LLMs' safe and ethical use in mission-critical IT governance? (Open Ended)                              \\
32. How can policies be developed to address the potential risks and challenges associated with the use of LLMs in security risk analysis? (Multiple Choice) \\
33. How can policies be developed to address the potential risks and challenges associated with the use of LLMs in security risk analysis? (Open Ended)      \\
34. What policies should be implemented to protect data privacy when using LLMs in mission-critical IT environments? (Multiple Choice)                       \\
35. What policies should be implemented to protect data privacy when using LLMs in mission-critical IT environments? (Open Ended)                            \\
36. What standards and guidelines would you recommend to ensure accountability and transparency in using LLMs for security risk analysis? (Multiple Choice)  \\
37. What standards and guidelines would you recommend to ensure accountability and transparency in using LLMs for security risk analysis? (Open Ended)       \\
38. How can policymakers engage with practitioners and researchers to create a balanced approach to integrating LLMs in mission-critical IT governance? (Multiple Choice) \\
39. How can policymakers engage with practitioners and researchers to create a balanced approach to integrating LLMs in mission-critical IT governance? (Open Ended) \\ \hline
\multicolumn{1}{c}{\textbf{Awareness and Categorization of LLMs in AI Regulations}}                                                                          \\ \hline
40. Are you aware of the recent "AI Act" by the European Union?                                                                                              \\
41. If you're familiar with the recent "AI Act," in which category would you place the use of large language models (LLMs) in the context of mission-critical applications?
\end{tabular}%
}
\end{table}
